Efficient Algorithms for Logistic Contextual Slate Bandits with Bandit Feedback

We study the Logistic Contextual Slate Bandit problem, where, at each round, an agent selects a slate of $N$ items from an exponentially large set (of size $2^{\Omega(N)}$) of candidate slates provided by the environment. A single binary reward, determined by a logistic model, is observed for the chosen slate. Our objective is to develop algorithms that maximize cumulative reward over $T$ rounds while maintaining low per-round computational costs. We propose two algorithms, Slate-GLM-OFU and Slate-GLM-TS, that accomplish this goal. These algorithms achieve $N^{O(1)}$ per-round time complexity via local planning (independent slot selections), and low regret through global learning (joint parameter estimation). We provide theoretical and empirical evidence supporting these claims. Under a well-studied diversity assumption, we prove that Slate-GLM-OFU incurs only $\tilde{O}(\sqrt{T})$ regret. Extensive experiments across a wide range of synthetic settings demonstrate that our algorithms consistently outperform state-of-the-art baselines, achieving both the lowest regret and the fastest runtime. Furthermore, we apply our algorithm to select in-context examples in prompts of Language Models for solving binary classification tasks such as sentiment analysis. Our approach achieves competitive test accuracy, making it a viable alternative in practical scenarios.

==> dtprsqbhrzmgzssxtywfnqcktqbmjtgr_5/arXiv_Sections_v2/Paper_Sections/conclusions.tex <==
\section{Conclusions}
\label{section:conclusions}

In this paper, we proposed three algorithms: \slateglincb, \slateglincbts, \slateglincbtsfixed\ for the slate bandit problem with logistic rewards. While the first two algorithms are designed for both the contextual and non-contextual settings, the third is designed particularly for the non-contextual setting. All our algorithms perform explore-exploit at the slot level, making their average per-round time complexity logarithmic in the number of candidate slates. By building on algorithms from \cite{Faury2022}, the average per-round time is also logarithmic in the number of rounds $T$. As a result, our algorithms run much faster than state-of-the-art logistic bandit algorithms (having $2^{\Omega(N)}$ per round time complexity). We also show that under a popular diversity assumption (Assumption \ref{assumption: diversity}), the consequences of which we validate in practice (Section \ref{appendix:empirical-validation}), \slateglincb\ and \slateglincbtsfixed\ achieve $\kappa$-independent  $\tilde{O}(\sqrt T)$ regret, making them both optimal and computationally efficient. 


==> dtprsqbhrzmgzssxtywfnqcktqbmjtgr_5/arXiv_Sections_v2/Paper_Sections/introduction.tex <==
\section{Introduction}
\label{section:introduction}
Online slate bandit problems provide a popular framework for modeling decision-making scenarios where multiple items must be selected in each round.  A slate consists of multiple slots, each with its own pool of candidate items, which may change over time. In each round, the learner selects one item per slot, thereby forming a slate.  A single reward drawn from a logistic model with unknown parameters is then received for the entire slate. The learner's objective is to adaptively optimize their slate selection policy to maximize the cumulative reward (or equivalently, minimize the cumulative regret) over time.  Online slate bandits naturally model various real-world applications.  A prominent example is landing page optimization \citep{Hill_2017}, where the goal is to optimize the selection of components for each part of a landing page to maximize conversions.  Another important application is the automatic optimization of advertising creatives \citep{Chen2021}, which requires advertisers to automatically compose ads from multiple elements, such as product images, text descriptions, and titles. Beyond these practical applications, slate bandits have been extensively studied in the academic literature, leading to the development of many interesting algorithms in diverse settings \citep{Kale2010, Dimakopoulou2019, Rhuggenaath2020}.

Although good progress has been made on a variety of online slate bandit settings, some significant challenges remain that limit the applicability of these algorithms. In applications such as those mentioned above, at each round, the learner has access to some contextual information (such as user query, user history, or demographics), which influences the set of available items per slot. To the best of our knowledge, the current literature focuses heavily on the non-contextual (fixed-arms\footnote{We use the terms arms and actions interchangeably.}) setting, i.e., they do not assume access to such contexts and therefore keep the set of items unchanged over time. Another limitation is that most of the prior work assumes that the reward of a slate is a (known or unknown) function of rewards of the items in the slate, which are themselves either adversarially chosen or are stochastic but disjoint from each other (i.e., each item's reward comes from a different distribution). This assumption neglects the inherent similarities between items.  A more realistic approach is to assume a unified parametric reward model shared across all slates.  This model allows the learner to leverage shared information, significantly simplifying the learning process.  Specifically, for binary rewards, models based on the logistic or probit function can effectively capture the reward structure.

A third, and equally important, limitation is the prevalent focus on the semi-bandit feedback setting.  This setting provides separate reward feedback for each item within a selected slate.  However, many practical applications (e.g., the ad creatives problem \citep{Chen2021}) offer only a single, slate-level reward (i.e., bandit feedback).  Although there are some methods for converting bandit feedback to semi-bandit feedback \citep{Dimakopoulou2019}, these are often heuristic and lack theoretical guarantees.  The item-level feedback in the semi-bandit setting facilitates per-slot exploration and exploitation, enabling the development of algorithms with $N^{O(1)}$ per-round complexity (e.g., \citep{Kale2010, Rhuggenaath2020}) by avoiding explicit iteration over the entire slate space.  It remains unclear if we can achieve a similar efficiency in the more challenging bandit feedback setting.  For example, directly applying state-of-the-art bandit algorithms \citep{Lattimore2020} to the slate bandit problem (by treating the set of slates as the arm-set) and selecting a slate by iterating through the $2^{\Omega(N)}$ sized set of all possible slates, results in exponential per-round time complexity.

Motivated by these challenges, our work introduces efficient and optimal algorithms for the logistic contextual slate bandit problem under bandit feedback, assuming time-varying item features and rewards generated from a global logistic model.  We now list our contributions.   

\subsection{Our Contributions}
\label{subsection:our-contributions}

\begin{enumerate}
    \item We propose two new algorithms \slateglincb\ and \slateglincbts\ that solve the logistic contextual slate bandit problem under bandit feedback. While \slateglincb\ is based on the OFU (Optimization in the Face of Uncertainty) paradigm, \slateglincbts\ follows the Thompson Sampling (TS) paradigm. Under a well-studied diversity assumption (Assumption \ref{assumption: diversity}), we prove that \slateglincb\ incurs a regret of $\Tilde{O}(dN\sqrt{T})$ with high probability. Here, the slate comprises $N$ slots, and each item in the slate is $d$-dimensional. Further, $T$ is the total number of rounds the algorithm is run for. Both algorithms explore and exploit at the slot level and thus have a per-round time complexity of $poly(N , \log T)$, making them feasible in practice.

    \item We also propose a fixed arm version \slateglincbtsfixed\ for the \slateglincbts\ algorithm in the non-contextual (fixed-arm) setting. Using an assumption similar to Assumption \ref{assumption: diversity}, we prove an $\tilde{O}(d^{3/2}N^{3/2} \sqrt{T})$ regret guarantee for \slateglincbtsfixed. Similar to \slateglincbts, \slateglincbtsfixed\ also explores and exploits at the slot level and has a per-round time complexity of $poly(N , \log T)$.
    
    \item We perform extensive experiments to validate the performance of our algorithms in both settings: contextual and non-contextual. Under a wide range of randomly selected instances, we see that \slateglincb\ incurs the least regret compared to all baselines. Also, \slateglincbts\ and  \slateglincbtsfixed\ are competitive with other state-of-the-art algorithms. We also evaluate the maximum and average per-round time complexity of our algorithms and compare them to the time complexities of our baselines. Our algorithms are exponentially (most of the time) faster than all baselines. 

    \item Finally, we use our algorithm \slateglincb\ to select in-context examples for tuning prompts of language models, applied to binary classification tasks. We perform experiments on two datasets \emph{SST2} and \emph{Yelp Review} and achieve a competitive test accuracy of $\sim 80\%$, making it a viable alternative in practical prompt-tuning scenarios.
\end{enumerate}


\subsection{Related Work}
\label{subsection:related-work}
Online slate bandits have received significant attention due to their wide applicability in applications such as recommendations and advertising \citep{Hill_2017, Chen2021, Dimakopoulou2019}; however, only a few theoretical studies provide regret guarantees \citep{Kale2010, Rhuggenaath2020}. While these papers make progress on the slate bandit problem, neither do they address the contextual setting, nor do they accommodate bandit feedback, which are the main motivations of our work. While analyzing the Thompson Sampling approach in \cite{Dimakopoulou2019} might be feasible, their algorithm assigns equal rewards to each slot to maintain slot-level policies for efficiency, and hence, proving optimal guarantees may still be difficult. However, we would like to acknowledge that in our experiments (Section \ref{section:experiments}), in the fixed-arm instances that we considered, we found their algorithm to be quite competitive with ours.

One way of achieving optimal regret guarantees for the slate bandit problem is to reduce it to the canonical logistic bandit problem by treating each candidate slate as a separate arm, and subsequently, use state-of-the-art algorithms, such as those in \citep{Faury2020, Abeille2021, Faury2022}. While these algorithms do achieve optimal ($\kappa$-free) regret, they would be rendered infeasible in practice. This is because the selection of an arm would require iterating through all the arms (which is a $2^{\Omega(N)}$ sized set), thereby incurring exponential time per round. Even though these algorithms are inefficient for the slate bandit problem, we utilize some of their key ideas with an efficient planning approach to design our algorithms. In Section \ref{section:experiments}, we demonstrate that our algorithms perform better than these state-of-the-art logistic bandit algorithms, both in regret and time complexity, when applied to a wide variety of slate bandit instances.


Recently, a large number of works \citep{Swaminathan2017, Kiyohara2024, Vlassis2021} have studied the slate bandit problem in the off-policy setting, wherein they utilize a dataset collected using some base policy to find optimal slate bandit policies. While these works have made significant progress both from the theoretical and practical sides, we focus on the online setting, and hence, they are not relevant to our work. 


% There exist other methods for Slate Bandits, such as \cite{Swaminathan2017}, who develop algorithms to learn offline-policies to choose slates, and \cite{Hill_2017}, who use the idea of hill-climbing to develop solutions for applications such as ad placements and landing page optimizations. The aim of this work to address all these limitations and develop computationally efficient algorithms for slate bandits with a logistic reward model in the Bandit Feedback setting.

==> dtprsqbhrzmgzssxtywfnqcktqbmjtgr_5/arXiv_Sections_v2/Paper_Sections/main-algorithm.tex <==
\clearpage
\section{\slateglincb}
\label{section:main-algo}




\begin{algorithm}[!ht] 
\caption{\texttt{Slate-GLM-OFU}}
\label{algo:batch_OFUL} 
    %\vspace{-3mm}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} Horizon $T$, probability of failure $\delta$, and upper bound on parameter norm $S$.

\STATE Initialize $\{\mathbf{W}_1^i\}_{i \in [N]} = \mathbf{I}_d$, $\mathbf{W}_1 = I_{dN}$, $\Theta_1 = \{\twonorm{\bm\theta} \leq S\}$, $\bm\theta_1 \in \Theta_1$, $\eta_t(\delta) = O(S^2Nd\log(t/\delta))$, and $ \H_1 = \emptyset$.
        
\FOR{each round $t \in [T]$}
\STATE For all slots $i \in [N]$, obtain the set of items $\mathcal{X}^i_t$ and find
$\mathbf{x}^i_t = \argmax_{\mathbf{x} \in \X^i_t} \mathbf{x}^\top \bm\theta_t^{i}+ \sqrt{\eta_t(\delta)} \matnorm{\mathbf{x}}{(\mathbf{W}_t^i)^{-1}}$.

\STATE Construct the slate $\mathbf{x}_t = (\mathbf{x}^1_t, \ldots, \mathbf{x}^N_t)$ and obtain the corresponding reward $y_t$.

\STATE Obtain $\bm\theta_{t+1}$, $\{\mathbf{W}_{t+1}^i\}_{i=1}^N$, $\Theta_{t+1}$, $\mathcal{H}_{t+1}$ by calling Algorithm \ref{algo:adaptive-updates} with inputs $\mathbf{x}_t$, $y_t$, $\bm\theta_t$, $\mathbf{W}_t$, $\{\mathbf{W}_{t}^i\}_{i=1}^N$, $\Theta_t$, $\mathcal{H}_t$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht] 
\caption{\texttt{ada-OFU-ECOLog-Updates}}
\label{algo:adaptive-updates} 
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} Slate $\mathbf{x}_t$, reward $y_t$, design matrices $\mathbf{W}_t, \{\mathbf{W}_{t}^i\}_{i=1}^N$, admissible set of parameters $\Theta_t$, set of indices $\mathcal{H}_t$.
\vspace{1mm}
\STATE Initialize $\gamma_t(\delta) = O(S^2Nd\log(t/\delta))$ and $\beta_t(\delta) = O(S^6Nd\log(t/\delta))$.
\vspace{1mm}
\STATE Compute $\bar{\bm\theta}_t$, $\bm\theta^0_t$, and $\bm\theta^1_t$ using 
\eqref{theta_bar} and \eqref{theta_u}.

\IF{$\dot{\mu}(\mathbf{x}_t^\top\bar{\bm\theta}_t) \leq 2\dot{\mu}(\mathbf{x}_t^\top\bm\theta^u_t)$ for $u \in \{0,1\}$}

\STATE Let $\bm\theta_{t+1}$ be solution of  \eqref{equation:optimization} up to precision $1/t$.

\STATE Update $\mathbf{W}_{t+1}^i \gets \mathbf{W}_t^i + \dot{\mu}(\mathbf{x}_t^\top\bm\theta_{t+1})\mathbf{x}_t^i{\mathbf{x}_t^i}^\top$, $\forall i\in [N]$.

\STATE Update $\mathbf{W}_{t+1} \gets \mathbf{W}_t + \dot{\mu}(\mathbf{x}_t^\top\bm\theta_{t+1})\mathbf{x}_t{\mathbf{x}_t}^\top$.

 \STATE Update $\H_{t+1} \gets \H_{t}$ and $\Theta_{t+1} \gets \Theta_t$.
 
 % \STATE $\mathcal{C}_{t+1}(\delta) = \{\lVert \bm\theta - \bm\theta_{t+1} \rVert^2_{\mathbf{W}_{t+1}} \leq \eta_t(\delta)\}$

\ELSE
\STATE Update $\H_{t+1} \gets \H_t \cup \{(\mathbf{x}_t, y_{t})\}$. 

\STATE Let $\bm\theta^\H_{t+1}$ be solution of \eqref{equation:optimization2} up to precision $1/t$.
                
\STATE Update $\mathbf{V}_{t}^\H \gets \kappa^{-1}\sum_{(\mathbf{x},y) \in \H_t}\mathbf{x}\mathbf{x}^\top + \gamma_t(\delta)\mathbf{I}_{Nd}$.
                
\STATE Update $\Theta_{t+1} \gets \cbrak{\matnorm{\bm\theta-\bm\theta^\H_{t+1}}{\mathbf{V}^\H_{t}}^2 \leq \beta_t(\delta)} \cap \Theta_1$.
\STATE Update $\bm\theta_{t+1} \gets \bm\theta_t$, $\mathbf{W}_{t+1} \gets \mathbf{W}_t$, and $\mathbf{W}_{t+1}^i \gets \mathbf{W}_t^i$, $\forall i\in [N]$.
\ENDIF
\STATE \textbf{return} $\bm\theta_{t+1}, \mathbf{W}_{t+1}, \{\mathbf{W}_{t+1}^i\}_{i=1}^N, \Theta_{t+1}, \mathcal{H}_{t+1}$.%, \mathcal{C}_{t+1}(\delta)$
\end{algorithmic}
\end{algorithm}

In this section, we present our first algorithm \slateglincb\ (Algorithm \ref{algo:batch_OFUL}) based on the OFU (Optimization in the Face of Uncertainty) paradigm \citep{Yadkori2011} used in bandit algorithms. At a high level, \slateglincb\ (along with sub-routine Algorithm \ref{algo:adaptive-updates}) builds upon the \adaofuecolog\ algorithm (Algorithm $2$ in \cite{Faury2022}) which achieves an optimal ($\kappa$-free) $O(\sqrt{T})$ regret guarantee for logistic reward models and incurs $O(K\log T)$ per round computational cost, where $K$ is the total number of actions to choose from. In the slate bandit setting, $K$ is exponential in $N$, the number of slots in the slate, making a direct application of \adaofuecolog\ infeasible when $N$ is large. To address this, \slateglincb\ selects an item for each slot independently, reducing the per-round computational cost to $N^{O(1)}$. Interestingly, despite choosing all the items comprising the slate independently, \slateglincb\ (via sub-routine Algorithm \ref{algo:adaptive-updates}) estimates only a single reward model using the slate-level reward feedback. This is a critical difference with respect to prior works on slate bandits with bandit feedback \citep{Dimakopoulou2019}, where the algorithm attributes the single slate-level reward feedback to individual items in the slate and estimates $N$ different reward models. 

\slateglincb\ takes as input $T$, the total number of rounds, $\delta$, the error probability, and $S$, a known upper bound for $\twonorm{\bm\theta^\star}$.
Similar to \adaofuecolog\ \citep{Faury2022}, \slateglincb\ maintains vectors $\bm\theta_t$, and sets $\Theta_t$ and $\mathcal{H}_t$. The vector $\bm\theta_t$ provides an estimate of $\bm\theta^\star$ during the $t^{th}$ round.
The set $\Theta_t \subseteq \Theta_1 =  \{\twonorm{\bm\theta}\leq S\}$ is the admissible set for the values of $\bm\theta_{t+1}$, and with high probability, contains the true reward parameter $\bm\theta^\star$ (See Proposition 7 in \cite{Faury2022}). In order to facilitate adaptivity, \adaofuecolog\  
introduced the sets $\mathcal{T}$ and $\mathcal{H}_t$, where $\mathcal{T}$ comprises all time rounds at which an inequality criterion (described in \emph{Step 4} of Algorithm \ref{algo:adaptive-updates}) fails, and $\mathcal{H}_t$ comprises the arm-reward pairs corresponding to these time rounds up to round $t$, i.e, $\mathcal{H}_t = \{(\mathbf{x}_s , y_s)\}_{s \in [t-1] \cap \mathcal{T}}$.
% We denote $\mathcal{T}$ to be the set of all time rounds at which this criterion fails. Similarly, following the notation in \cite{Faury2022}, $\mathcal{H}_t$ denotes the set comprising all arm-reward pairs $\{\mathbf{x}_s , y_s\}_{s \in [t-1] \cap \mathcal{T}}$ corresponding to the rounds at which the 
% introduced the set $\mathcal{H}_t$, which comprises all arm-reward pairs corresponding to the time-steps 

% comprising arm-reward pairs $\{(\mathbf{x}_s, y_s(\mathbf{x}_s))\}_{s \leq t}$ corresponding to the time-steps at which an inequality criterion (described in \emph{Step 4} of Algorithm \ref{algo:adaptive-updates}) fails. 
In addition to these, to enable efficient per-round computation of parameter estimates, \adaofuecolog\ also introduced the matrix $\mathbf{W}_t$ as an on-policy proxy for the concentration matrix $\mathbf{H}_t$, where $\mathbf{H}_t$ and $\mathbf{W}_t$ are defined as
\[
    \mathbf{H}_t =  \mathbf{I}_{Nd} + \sum_{s \in [t-1] \setminus \mathcal{T}}\dot{\mu}(\mathbf{x}_s^\top\bm\theta^\star)\mathbf{x}_s\mathbf{x}_s^\top, \quad \mathbf{W}_t= \mathbf{I}_{Nd} + \sum_{s \in [t-1] \setminus \mathcal{T}} \dot{\mu}(\mathbf{x}_{s}^\top \bm\theta_{s+1})\mathbf{x}_{s}\mathbf{x}_{s}^\top.
\]


% $\mathbf{W}_t= \lambda\mathbf{I} + \sum_{s=1}^{[t-1]\setminus \mathcal{H}_t} \dot{\mu}(\mathbf{x}_{s}^\top \bm\theta_{s+1})\mathbf{x}_{s}\mathbf{x}_{s}^\top$ as an on-policy proxy for the \emph{concentration matrix} $\mathbf{H}_t = \lambda\mathbf{I} + \sum_{s=1}^{[t-1]\setminus \mathcal{H}_t}\dot{\mu}(\mathbf{x}_s^\top\bm\theta^\star)\mathbf{x}_s\mathbf{x}_s^\top$, 
 In \slateglincb, we additionally maintain $N$ other such matrices corresponding to each of the $N$ slots. The $i^{th}$ matrix, denoted by $\mathbf{W}^i_t$, helps in the explore-exploit trade-off while selecting an item for the $i^{th}$ slot. This matrix $\mathbf{W}^i_t$ is defined as
 \[
    \mathbf{W}_t^i =  \mathbf{I}_{d} + \sum_{s \in [t-1]\setminus \mathcal{T}} \dot{\mu}(\mathbf{x}_{s}^\top \bm\theta_{s+1})\mathbf{x}_{s}^i{\mathbf{x}_{s}^i}^\top.
 \]
 
Next, we go through the steps of \slateglincb\ (Algorithm \ref{algo:batch_OFUL}) and its sub-routine (Algorithm \ref{algo:adaptive-updates}) to provide a more detailed explanation.
\emph{Steps 3-7} (Algorithm \ref{algo:batch_OFUL}) is where \slateglincb\ significantly differs from \adaofuecolog. Instead of obtaining the set of arm features $\mathcal{X}_t$ (in our case, slates) directly from the environment (as in \adaofuecolog), \slateglincb\ receives $N$ different sets of items $\mathcal{X}_t^i,$ for each slot $i\in [N]$. Then, it picks an item $\mathbf{x}_t^i \in \mathcal{X}_t^i$, using the optimistic rule mentioned in \emph{Step 4} (Algorithm \ref{algo:batch_OFUL}). Note that the underlying optimization problem for slot $i$ only requires the candidate items in $\X_t^i$ and the components $\bm\theta_t^i$ of $\bm\theta_t$ corresponding to the $i^{th}$ slot, and hence, can be solved independently and in parallel for all slots. A core technical part of our regret guarantee (Theorem \ref{theorem: Regret OFUL}) is to demonstrate how the independent selection of items at the slot-level leads to optimal selection at the slate-level. Essentially, we can show that, under our diversity assumption (Assumption \ref{assumption: diversity}), with high probability, the positive definite matrices $\mathbf{W}_t$ and $\textrm{diag}(\mathbf{W}_t^1,\ldots, \mathbf{W}_t^N)$ are multiplicatively equivalent, i.e, for some $c^\prime \in (0,1)$,
\[
    (1-c^\prime) \textrm{diag}(\mathbf{W}_t^1,\ldots, \mathbf{W}_t^N) \preceq \mathbf{W}_t \preceq (1+c^\prime) \textrm{diag}(\mathbf{W}_t^1,\ldots, \mathbf{W}_t^N).
\]
This multiplicative equivalence allows us to show that for all slates $\mathbf{x}_t = (\mathbf{x}^1_t , \ldots , \mathbf{x}^N_t)$, 
\[
    \matnorm{\mathbf{x}_t}{\mathbf{W}_t\inv} \leq  \frac{1}{1-c^\prime} \sum_{i\in [N]}\matnorm{\mathbf{x}_t^i}{(\mathbf{W}_t^i)\inv},
\]
i.e, the quantities $\matnorm{\mathbf{x}_t}{\mathbf{W}_t\inv}$ and $\sum_{i\in [N]}\matnorm{\mathbf{x}_t^i}{(\mathbf{W}_t^i)\inv}$ are also multiplicatively equivalent. We then exploit this observation to convert the slate-level optimistic selection rule into an equivalent optimistic selection rule for each slot.
In \emph{Step 5} (Algorithm \ref{algo:batch_OFUL}), we select the slate $\mathbf{x}_t = (\mathbf{x}_t^1, \ldots, \mathbf{x}_t^N)$, yielding a reward $y_t$. At this point, \slateglincb\ calls a sub-routine described in Algorithm \ref{algo:adaptive-updates} which updates the parameters $\bm\theta_t$, $\mathbf{W}_t$, $(\mathbf{W}_t^1, \ldots, \mathbf{W}_{t}^N)$, $\Theta_t$, and $\mathcal{H}_t$. The update rules in Algorithm \ref{algo:adaptive-updates} largely follow the one in \adaofuecolog, which is based on the following inequality criterion:
\begin{equation}
\dot{\mu}(\mathbf{x}_t^\top \bar{\bm\theta}_t) \leq 2 \min\{\dot{\mu}(\mathbf{x}_t^\top \bm\theta^0_{t}), \dot{\mu}(\mathbf{x}_t^\top \bm\theta^1_{t})\}.
\label{equation:adaptivity-criterion}
\end{equation}
Here $\bar{\bm\theta}_t, \bm\theta_t^0, \bm\theta_t^1 \in \R^{dN}$, are $\mathcal{F}_t$-adapted parameters that enable adaptivity. They are obtained as follows:
\begin{equation}
    \bar{\bm\theta}_t = \argmin\limits_{\bm\theta \in \Theta_t} \sbrak{\eta \matnorm{\bm\theta - \bm\theta_t}{\mathbf{W}_t}^2 + \ell(\inner{\mathbf{x}_t}{\bm\theta} , 0) + \ell(\inner{\mathbf{x}_t}{\bm\theta} , 1)},
    \label{theta_bar}
\end{equation}

\begin{equation}
    {\bm\theta}^u_t = \argmin\limits_{\bm\theta \in \Theta_t} \sbrak{\eta \matnorm{\bm\theta - \bm\theta_t}{\mathbf{W}_t}^2 + \ell(\inner{\mathbf{x}_t}{\bm\theta} , u)},
    \label{theta_u}
\end{equation}
where $\ell(\mathbf{x},y) = -y\log \mu(\mathbf{x}) - (1-y) \log (1-\mu(\mathbf{x}))$ is the cross-entropy loss and $\eta = (2+diam(\Theta_t))^{-1}$. When the inequality in \eqref{equation:adaptivity-criterion} is true, the algorithm updates $\bm\theta_{t}, \mathbf{W}_t$ and $\mathbf{W}_t^i$ ($i\in [N]$) as per \emph{Steps 5-7} (Algorithm \ref{algo:adaptive-updates}). First, in \emph{Step 5}, $\bm\theta_{t+1}$ is computed by solving the following optimization problem up to a precision of $1/t$:
\begin{equation}
    \label{equation:optimization}
    \bm\theta_{t+1} = \arg \min\limits_{\Theta_t} \sbrak{\eta\matnorm{\bm\theta - \bm\theta_t}{\mathbf{W}_t}^2 + \ell(\inner{\mathbf{x}_t}{\bm\theta} , y_{t})}.
\end{equation}
Next, $\mathbf{W}_t^i$ ($i\in [N]$) and $\mathbf{W}_t$ are updated in \emph{Step 6} and \emph{Step 7}  as per their definitions provided earlier. When the inequality in \eqref{equation:adaptivity-criterion} does not hold, the algorithm instead updates $\mathcal{H}_t$ and $\Theta_t$ as described in \emph{Steps 10-13} (Algorithm \ref{algo:adaptive-updates}). In \emph{Step 10}, $\mathcal{H}_t$ is updated to $\mathcal{H}_{t+1}$ by adding the arm-reward pair $(\mathbf{x}_t, y_t)$ to it. Using $\mathcal{H}_{t+1}$, in \emph{Step 11}, the algorithm recomputes the estimate of $\bm\theta^\star$, given by $\bm\theta_{t+1}^\mathcal{H}$, by minimizing the regularized cross-entropy loss (up to a precision $1/t$) as follows:
\begin{equation}
\label{equation:optimization2}
    \bm\theta^\H_{t+1} = \argmin\sum\limits_{(\mathbf{x},y) \in \H_{t+1}} \ell(\inner{\mathbf{x}}{\bm\theta} , y) + \gamma_t(\delta)\twonorm{\bm\theta}^2.
\end{equation}
Using this estimate, and a design matrix $\mathbf{V}_t^{\mathcal{H}}$ (computed in \emph{Step 12}), in \emph{Step 13}, the set $\Theta_t$ is updated to $\Theta_{t+1}$ by taking an intersection between a confidence set of radius $\beta_t(\delta)= O(dN\log (t/\delta))$ around the new estimate $\bm\theta_{t+1}^{\mathcal{H}}$ (that contains the optimal parameter $\bm\theta^\star$ with high probability) and the initial set $\Theta_1 = \{\twonorm{\bm\theta}\leq S\}$. Updating $\Theta_t$ when the inequality in \eqref{equation:adaptivity-criterion} fails ensures that \eqref{equation:adaptivity-criterion} is more likely to succeed in the future.
In Lemma \ref{lemma: warmup}, we show that $|\mathcal{H}_T| = \tilde O(\kappa d^2 N^2 S^6)$. The rounds corresponding to $\mathcal{H}_T$, therefore, incur at most $\tilde O(\kappa d^2 N^2 S^6)$ regret. 

In Theorem \ref{theorem: Regret OFUL}, we provide a regret guarantee for \slateglincb\ and present its proof in Appendix \ref{appendix: proof_regret_oful}.

\begin{theorem}[Regret of \slateglincb]
\label{theorem: Regret OFUL}
Let $\mathcal{T} = \{s\in [T]: (\mathbf{x}_s, y_s)\in \mathcal{H}_T\}$, i.e, the set of rounds up till round $T$ where the inequality condition in \eqref{equation:adaptivity-criterion} fails. Also, let $\mathbf{x}_{\star, t} = \argmax_{\mathbf{x}\in \mathcal{X}_t} \mu(\mathbf{x}^\top\bm\theta^\star)$, be the optimal slate at round $t\in [T]$. Under the diversity assumption (Assumption \ref{assumption: diversity}), at the end of $T$ rounds, the regret incurred by \slateglincb, denoted by $R(T)$, can be bounded as
\[
R(T) = \tilde O\left(SdN\sqrt{\sum\limits_{t\notin \mathcal{T}} \dot{\mu}(\mathbf{x}_{\star, t}^\top \bm\theta^\star)} + S^6 d^2 N^2 \kappa \right).
\] 
\end{theorem}


\textbf{Remark: }Let $\mathcal{T}$ be as defined in Theorem \ref{theorem: Regret OFUL}. The per-round time complexity of \slateglincb\ is $O(d^2 N^2 \log^2 t)$ for rounds $t\in [T]\setminus \mathcal{T}$, and, $O(dNt)$ for rounds $t\in \mathcal{T}$. However, from Lemma \ref{lemma: warmup}, we have that the $O(dNt)$ per-round complexity is incurred only for $|\mathcal{T}| = \tilde{O}(\kappa d^2 N^2 S^6)$ rounds.



\section{\slateglincbts}
\label{section:TS}
In this section, we present our second algorithm, \slateglincbts\ (Algorithm \ref{algo:TS}) based on the Thompson Sampling paradigm \citep{Thompson1933, Russo2018} used in bandit algorithms. \slateglincbts\ builds upon the \tsecolog\ algorithm (Algorithm $3$ in Appendix $D.2$, \cite{Faury2022}) while adapting to the changing action sets using the update strategy in Algorithm \ref{algo:adaptive-updates}. \tsecolog\ adapts the Linear Thompson Sampling algorithm from \cite{Abeille2017} that perturbs the estimated parameter vector by adding an appropriately transformed noise vector sampled from a suitable multivariate distribution $\mathcal{D}^{TS}$ (refer Figure 1 in \cite{Abeille2017}) satisfying certain properties (Definition \ref{def: D_TS}). Following this, the optimal action (in our case, slate) with respect to the new perturbed parameter vector is chosen. While \tsecolog\ achieves an optimal regret guarantee of $O(\sqrt{T})$ for fixed action sets and a logistic reward model, similar to \adaofuecolog\ , it also incurs per-round computational cost proportional to the number of actions $K$ (recall $K = 2^{\Omega(N)}$ in our setting), since it selects arms at the slate-level. To circumvent this exponential time-complexity, \slateglincbts\ operates at the slot-level. For each slot $i\in [N]$, it perturbs the components of the estimated parameter vector (corresponding to the $i^{th}$ slot) using a noise vector sampled independently of all other slots. Then, it chooses the optimal item from each slot independent of the others, hence, choosing the slate with $N^{O(1)}$ per-round time complexity. While the items for each slot are determined independently, similar to \slateglincb, \slateglincbts\ also estimates a single reward model and updates the parameter vector for this model jointly using the slate-level reward $y_t$, by employing the update strategy in Algorithm \ref{algo:adaptive-updates}. 

\slateglincbts\ takes as inputs the time horizon $T$, the error probability $\delta$, $S$, a known upper bound for $\twonorm{\bm\theta^\star}$, and a multivariate distribution satisfying the properties stated in (Definition $1$, \cite{Abeille2017}), denoted by $\mathcal{D}^{TS}$.
During the course of the algorithm, \slateglincbts\ maintains vectors $\bm\theta_t$, matrices $\mathbf{W}_t$, $\mathbf{W}_t^i$ ($i\in [N]$) and sets $\Theta_t, \mathcal{H}_t$ with exactly the same definitions as in \slateglincb.


Next, we go through the steps of \slateglincbts\ (Algorithm \ref{algo:TS}).
\emph{Steps 3-10} is where \slateglincbts\ differs significantly from \tsecolog. Instead of getting the set of arm features $\mathcal{X}_t$ (in our case, slates) directly from the environment (as in \tsecolog), \slateglincbts\ receives $N$ different sets of items $\mathcal{X}_t^i, i\in [N]$ in \emph{Step 4}.
While \tsecolog\ samples a noise vector $\bm\eta\in \R^{dN}$ from $\mathcal{D}^{TS}$ and perturbs the estimated parameter vector $\bm\theta_t$ \
by adding (a scalar multiple of) $({\mathbf W_t})^{-1/2} \bm\eta$, \slateglincbts\ samples $N$ \textrm{i.i.d} vectors $\bm\eta_1,\ldots, \bm\eta_N$ and perturbs each component of $\bm\theta_t = (\bm\theta^1_t , \ldots , \bm\theta^N_t)$ as 
\[
    \tilde{\bm\theta}^i_t = \bm\theta^i_t + \eta_t(\delta) (\mathbf{W}^i_t)^{-\frac{1}{2}}\bm\eta^i,
\]
i.e, the $i^{th}$ component of $\bm\theta_t$ is perturbed by adding to it (a scalar multiple of) $({\mathbf W_t^i})^{-1/2} \bm\eta_i$ (\emph{Step 7} and \emph{8}).
% $\bm\theta_t^i$ of $\bm\theta_t = (\bm\theta_t^1, \ldots, \bm\theta_t^N)$ (corresponding to the item features in the $i^{th}$ slot) to $\tilde{\bm\theta}_t^i \in \R^d$ by adding to it (a scalar multiple of) $({\mathbf W_t^i})^{-1/2} \bm\eta_i$ (\emph{Step 7} and \emph{8}).
Thus, by perturbing $\bm\theta_t$ , the algorithm performs rejection sampling till the perturbed vector $\tilde{\bm\theta}_t$ belongs to the set of admissible parameters $\Theta_t$.
% The algorithm continues to perform rejection samplingsample these noise vectors until the perturbed vector $\tilde{\bm\theta}_t = (\tilde{\bm\theta}_t^1, \ldots, \tilde{\bm\theta}_t^N)$ belongs to the admissible set $\Theta_t$. 
Then, in \emph{Step 11}, it picks the item $\mathbf{x}_t^i \in \mathcal{X}_t^i$, that is optimal with respect to the perturbed parameter vector $\tilde{\bm\theta}_t^i$. Note that, the underlying optimization problem for slot $i$ only requires the candidate items in $\X_t^i$ and the perturbed vectors $\tilde{\bm\theta}_t^i$, and hence, can be solved independently and in parallel for all slots. In \emph{Step 12}, we select the slate $\mathbf{x}_t = (\mathbf{x}_t^1, \ldots, \mathbf{x}_t^N)$, yielding a reward $y_t$. At this point, \slateglincb\ calls a sub-routine described in Algorithm \ref{algo:adaptive-updates} which performs updates to $\bm\theta_t$, $\mathbf{W}_t$, $(\mathbf{W}_t^1, \ldots, \mathbf{W}_{t}^N)$, $\Theta_t$, $\mathcal{H}_t$. 

Now, we make a few additional remarks about \slateglincbts\ below.
\begin{algorithm}[!ht] 
\caption{\texttt{Slate-GLM-TS}}
\label{algo:TS} 
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} Horizon $T$, probability of failure $\delta$, upper bound on parameter norm $S$, and a distribution $\mathcal{D}^{TS}$.

\STATE Initialize $\{\mathbf{W}^i_1\}_{i \in [N]} = \mathbf{I}_d$, $\mathbf{W}_1 = I_{dN}$, $\Theta_1 = \{\twonorm{\bm\theta}\leq S\}$, $\bm\theta_1 \in \Theta_1$, $\eta_t(\delta) = O(S^2Nd\log(t/\delta))$, and $ \H_1 = \emptyset$.
        
\FOR{each round $t \in [T]$}
\STATE Obtain the set of items $\mathcal{X}^i_t$, $\forall i \in [N]$.
\STATE Set reject = True.
\WHILE{reject}
    \STATE Sample $\mathbf{\eta}^{1}, \ldots, \mathbf{\eta}^N \overset{\mathrm{iid}}{\sim} \mathcal{D}^{TS}$. 
    \STATE Define $\tilde{\bm\theta}^{i}_t = \bm\theta^{i}_t + \eta_t(\delta)(\mathbf{W}_t^i)^{-1/2}\mathbf{\eta}^{i}$, $\forall i\in [N]$.
    \STATE If $\tilde{\bm\theta}_t = (\tilde{\bm\theta}^{1}_t , \ldots  \tilde{\bm\theta}^{N}_t) \in \Theta_t$, set reject = False.
\ENDWHILE
\STATE For each $i\in [N]$, find item $\mathbf{x}^i_t = \argmax_{\mathbf{x} \in \X^i_t} \inner{\mathbf{x}}{\tilde{\bm\theta}^{i}_t}$.

\STATE Select slate $\mathbf{x}_t = (\mathbf{x}^1_t, \ldots, \mathbf{x}^N_t)$ and obtain corresponding reward $y_t$.

\STATE Obtain $\bm\theta_{t+1}$, $\mathbf{W}_{t+1}$, $(\mathbf{W}_{t+1}^1, \ldots, \mathbf{W}_{t+1}^N)$, $\Theta_{t+1}$, $\mathcal{H}_{t+1}$ by calling Algorithm \ref{algo:adaptive-updates} with inputs $\mathbf{x}_t$, $y_t$, $\bm\theta_t$, $\mathbf{W}_t$, $(\mathbf{W}_t^1, \ldots, \mathbf{W}_{t}^N)$, $\Theta_t$, $\mathcal{H}_t$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

\textbf{Remark: }It's easy to see that the per-round time complexity of \slateglincbts\ is $N(d\log T)^{O(1)}$. This is significantly lower than that of \texttt{TS-ECOLog}, which has time complexity exponential in $N$. The improvement comes as a result of the slot-level selection in \slateglincbts. This, along with the efficient estimation of $\bm\theta_t$ in Algorithm \ref{algo:adaptive-updates}, ensures that the algorithm has low per-round time complexity, making it useful in practical scenarios. This is validated by our Synthetic experiments in Section \ref{section:experiments}. Also, in several different instances, we observe that the regret incurred by \slateglincbts\ is competitive (and in most cases, better) than other baselines. 
% In fact, in many experiments, it was only second to \slateglincb\ which had the lowest regret. 
Even though we do not provide a theoretical guarantee for the regret of \slateglincbts, in Appendix \ref{appendix: regret_proof_TS}, we provide a fixed-arm version for \slateglincbts\ called \slateglincbtsfixed. Like \tsecolog\ , \slateglincbtsfixed\ operates in the non-contextual setting, i.e., the action features (in our case, set of slates) remain fixed over time. It combines a short warm-up procedure from \tsecolog\ and the slot-level selection technique from \slateglincbts\, which results in a per-round time complexity that grows as $poly(N)$. Under the diversity assumptions (Assumption \ref{assumption: diversity}), we utilize a multiplicative equivalence between  $\mathbf W_t$ and $diag(\mathbf W_t^1, \ldots , \mathbf W_t^N)$ (similar to the one described in Section \ref{section:main-algo}) to prove an optimal $O(\sqrt{T})$ regret guarantee on the number of rounds $T$. For brevity, we discuss details of \slateglincbtsfixed\ (Algorithm \ref{algo:TS-Fixed}) and its regret guarantee (Theorem \ref{theorem:TS}) in Appendix \ref{appendix: regret_proof_TS}.



==> dtprsqbhrzmgzssxtywfnqcktqbmjtgr_5/arXiv_Sections_v2/Paper_Sections/notations.tex <==
\section{Preliminaries}
\label{section:preliminaries}
In this section, we define the notations used in the paper. Following this, we
formulate the Slate Bandits problem and present the assumptions that enable us to prove the regret guarantees stated in Theorem \ref{theorem: Regret OFUL} and Theorem \ref{theorem:TS}.

\paragraph{Notations:} We denote the set $\cbrak{1,2\ldots,N}$ as $\sbrak{N}$. Unless otherwise specified, all vectors, matrices, and sets are represented using bold lower-case, bold upper-case, and calligraphic upper-case or Greek letters, respectively. 
For any matrix $\mathbf{A}$, we denote its minimum and maximum eigenvalues as $\lambda_{\min}(\mathbf{A})$ and $\lambda_{\max}(\mathbf{A})$ respectively. 
We write $\mathbf{A}\mgeq 0$, if all the eigenvalues of the matrix $\mathbf{A}$ are non-negative (i.e, it is positive semi-definite), and $\mathbf{A}\mgeq \mathbf{B}$, if $\mathbf{A}-\mathbf{B}\mgeq 0$. For a positive semi-definite matrix $\mathbf{A}$, we define the norm of a vector $\mathbf{x}$ with respect to $\mathbf{A}$ as $\matnorm{\mathbf{x}}{\mathbf{A}} = \sqrt{\mathbf{x}^\top{\mathbf{A}}\mathbf{x}}$ and the spectral norm of $\mathbf{A}$ as $\twonorm{\mathbf{A}} = \sqrt{\eigmax{\mathbf{A}^\top\mathbf{A}}}$. We use $\mathbf{I}_{m}$ and $\mathbf{0}_{m}$ to denote the $m\times m$ identity and zero matrices respectively. When the dimension $m$ is clear from the context, we use $\mathbf{I}$ and $\mathbf{0}$ instead. The symbols $\P$ and $\E$ denote probability and expectation, respectively. For a set $\mathcal{X} \subseteq \R^m$, we define the diameter of $\mathcal{X}$ as $diam(\mathcal{X}) = \max\limits_{\mathbf{x}_1 ,\mathbf{x}_2 \in \mathcal{X}} \lVert \mathbf{x}_1 - \mathbf{x}_2 \rVert_2$. Also, for two sets $\mathcal{A}$ and $\mathcal{X}$, such that $\mathcal{A},\mathcal{X} \subseteq \R^m$, the diameter of $\mathcal{X}$ with respect to $\mathcal{A}$ is defined as $diam_{\mathcal{A}}(\mathcal{X}) = \max\limits_{\mathbf{a} \in \mathcal{A}} \max\limits_{\mathbf{x}_1 , \mathbf{x}_2 \in \mathcal{X}} \lvert \mathbf{a}^\top (\mathbf{x}_1 - \mathbf{x}_2) \rvert$. Finally, throughout the paper, we use $\tilde{O}(.)$ to suppress logarithmic factors.

\subsection{Slate Bandits}
In the Slate Bandit problem, a learner interacts with the environment over $T$ rounds. At each round $t\in [T]$, the learner is presented with $N$ finite sets $\mathcal{X}^i_t$ $(\subset \R^{d}), i\in [N]$, of \emph{items} and is expected to select one item (say $\mathbf{x}^i_t$) from each $\mathcal{X}^i_t$. Based on the selected $N$-tuple $\mathbf{x}_t = (\mathbf{x}^1_t,\ldots,  \mathbf{x}^N_t)$ (called a ``slate''), the learner receives a stochastic binary reward $y_t(\mathbf{x}_t)$. The goal of the learner is to select a sequence of slates $\{\mathbf{x}_t\}_{t \in [T]}$ such that her expected regret
\[
Regret(T) = \sum\limits_{t=1}^T \bigg\{\max_{\mathbf{x}\in \mathcal{X}_t}\E[y_t(\mathbf{x})] - \E[y_t(\mathbf{x}_t)] \bigg\}
 \]
is minimized\footnote{We also use $R(T)$ for shorthand.}. Here, $\mathcal{X}_t$ denotes the set $\mathcal{X}^1_t\times\ldots\times \mathcal{X}^N_t$ of all possible slates at round $t$. When the chosen slate $\mathbf{x}_t$ is clear from the context, for simplicity, we will denote $y_t(\mathbf{x}_t)$ as $y_t$. For simplicity, we say that the slate $\mathbf{x}_t$ comprises $N$ ``slots'', and the item $\mathbf{x}_t^i$ is placed in slot $i$ in the slate. 


% In this work, we consider two well-known settings: $(a)$ \textbf{Stochastic Contextual} and $(b)$ \textbf{Non-Contextual} (also known as the Fixed-Arm setting). In the second setting, we assume $\mathcal{X}_t^i$ remains fixed over time. Thus, in this setting, for simplicity, we denote $\mathcal{X}_t^i$ by $\mathcal{X}^i$.

In this work, we consider two well-known settings:
\begin{enumerate}
    \item \textbf{Stochastic Contextual Setting}: In this setting, at each round $t \in [T]$ and for each slot $i \in [N]$, we assume that the set $\mathcal{X}^i_t$ is constructed by sampling from a distribution $\mathcal{D}_i$, in an $\mathrm{i.i.d}$ fashion. Moreover, $\mathcal{X}_t^i$ and $\mathcal{X}_s^j$ are sampled independently of one another, for all $s,t \in [T]$ and $i,j \in [N]$. 
    \item \textbf{Non-Contextual Setting}: This setting is also known as the Fixed-Arm Setting.  Here, the item-sets $\mathcal{X}_t^i$ for all slots $i \in [N]$ remain fixed over time. Thus, for simplicity, we denote $\mathcal{X}_t^i$ by $\mathcal{X}^i$ for all $t \in [T]$.
\end{enumerate}

\paragraph{Logistic rewards:}In this paper, we assume that the binary reward variable $y_t$ comes from a Logistic Model. Therefore, $
\P[y_t=1 \mid \mathbf{x}_t] = \mu(\mathbf{x}_t^\top\mathbf\theta^\star)$,
where $\mu:\R\rightarrow\R$ is the logistic function, i.e., $\mu(a) = 1/(1+\exp(-a))$, and
$\mathbf{\theta}^\star\in \R^{dN}$ is an unknown $dN$-dimensional parameter vector. Similar to prior works on Logistic bandits \citep{Faury2020, Abeille2021, Faury2022}, we assume that $\twonorm{\mathbf\theta^\star}\leq S$, where $S$ is known to the learner\footnote{Often, an upper bound on $S$ suffices.}, and $\twonorm{\mathbf{x}^i}\leq 1/\sqrt{N}$, for all $\mathbf{x}^i\in \mathcal{X}_t^i$, $i\in [N], t\in [T]$\footnote{This implies the usual assumption $\twonorm{\mathbf{x}}\leq 1$ for all $\mathbf{x}\in \mathcal{X}_t$.}. 

Recent logistic bandit literature \citep{Filippi2010, Faury2020, Abeille2021, Faury2022} also identifies a critical parameter $\kappa$ that captures the non-linearity of the reward for the given problem instance, defined as follows:

\begin{equation}
    \kappa = \max_{t\in [T]} \; \max_{\substack{\mathbf{x} \in \X_t \\ \mathbf\theta\in\Theta}} \frac{1}{\dot{\mu}(\mathbf{x}^\top \mathbf\theta)},
    \label{eqn:kappa}
\end{equation}

where $\Theta =\{\twonorm{\mathbf\theta}\leq S\} \subset \R^{dN}$. The parameter $\kappa$ can be intuitively seen as the mismatch between the true reward function and a linear approximation of the same. It is well known that $\kappa$ grows exponentially with the diameter of $\Theta$ \cite{Faury2020}, and hence, developing algorithms with regret independent of $\kappa$ is ana ctive area of research that has gained significant attention \citep{Faury2020, Abeille2021, Faury2022, Sawarni2024}.
% Recently, developing algorithms with regret independent of $\kappa$ has gained significant attention \citep{Faury2020, Abeille2021, Faury2022, Sawarni2024} and is an active area of research. 
We refer the reader to Section 2 of \cite{Faury2020} for a thorough discussion on $\kappa$ and its implications on regret analysis. 

We now describe a key assumption that enables us to design algorithms with low per-round computational complexity and strong regret guarantees (Theorem \ref{theorem: Regret OFUL} in Section \ref{section:main-algo} and Theorem \ref{theorem:TS} in Appendix \ref{appendix:ts-algos}). 

\begin{assumption}
    (\textbf{Diversity Assumption}) Let $\mathcal{F}_t$ be the sigma algebra generated by $\{\mathbf{x}_1, y_1, \ldots, \mathbf{x}_{t-1}, y_{t-1}\}$ and $\emptyset = \mathcal{F}_0\subset\mathcal{F}_1\subset \ldots \mathcal{F}_T$, be the associated filtration. For each $i\in [N]$ and $t\in [T]$, we assume that,
\[
\E[\mathbf{x}_t^i\mid \mathcal{F}_t] = \mathbf{0} \hspace{1em}\text{and} \hspace{1em} \E[\mathbf{x}_t^i{\mathbf{x}_t^i}^\top \mid \mathcal{F}_{t}] \mgeq \rho \kappa \mathbf{I},
\]

where $\rho >0$ is a fixed constant and $\kappa$ is the non-linearity parameter defined earlier in \eqref{eqn:kappa}.
\label{assumption: diversity}
\end{assumption}

\textbf{Remarks on Assumption \ref{assumption: diversity}: }
The diversity assumption intuitively ensures that for each slot $i\in [N]$ and round $t\in [T]$, the item features $\mathbf{x}_t^i$ selected by the algorithm are sufficiently ``diverse'', i.e., the expected matrix $\E[\mathbf{x}_t^i{\mathbf{x}_t^i}^\top \mid \mathcal{F}_{t}]$ is full-rank and has sufficiently large eigenvalues. In our proofs, we first use this assumption to prove that, with high probability, the minimum eigenvalue of certain design matrices used in our algorithms (Algorithms \ref{algo:batch_OFUL}, \ref{algo:TS}, \ref{algo:TS-Fixed}) grows (sufficiently) linearly with time. We denote these design matrices as $\mathbf{W}^i_t$ and define them as
\[
\mathbf{W}_t^i = \mathbf{I}_d + \sum_{s\in [t-1]\setminus \mathcal{T}}\dot{\mu}(\mathbf{x}_s^\top\mathbf{\theta}_{s+1})\mathbf{x}_s^i{\mathbf{x}_s^i}^\top \; \forall i \in [N],
\]
where $\mathcal{T} \subset [T]$.
% used by our algorithms (Algorithms \ref{algo:batch_OFUL}, \ref{algo:TS}, \ref{algo:TS-Fixed}) grows (sufficiently) linearly with $t$.
In particular, in Lemma \ref{lemma: min_eig_design}, we show that
\[ 
\P\cbrak{\lambda_{min}(\mathbf{W}_t^i) \geq 1 + c\rho |[t-1]\setminus \mathcal{T}|} \geq 1 - \delta,
\]
% (Lemma \ref{lemma: min_eig_design}, Appendix \ref{appendix:general}) $
for a fixed constant $c \in (0,1)$. Then, in Lemma \ref{lemma: ineq on W} and Lemma \ref{lemma:multiplicative-equivalence}, we critically utilize this fact 
% (Lemma \ref{lemma: ineq on W}, Appendix \ref{appendix: proof_regret_oful} and Lemma \ref{lemma:multiplicative-equivalence}, Appendix \ref{appendix: general_lemmas_ts}) 
to prove a multiplicative equivalence between a block diagonal matrix comprising $\mathbf{W}^i_t$ for all slots $i \in [N]$, and a similarly defined slate-level design matrix
$\mathbf{W}_t = \mathbf{I}_{Nd} + \sum_{s\in [t-1]\setminus \mathcal{T}}\dot{\mu}(\mathbf{x}_s^\top\mathbf{\theta}_{s+1})\mathbf{x}_s\mathbf{x}_s^\top$, i.e, we show that for some $c^\prime \in (0,1)$
\[
    (1-c^\prime) \textrm{diag} (\mathbf{W}^1_t , \ldots , \mathbf{W}^N_t) \preceq \mathbf{W}_t \preceq (1+c^\prime) \textrm{diag} (\mathbf{W}^1_t , \ldots , \mathbf{W}^N_t).
\]
This multiplicative equivalence allows us to replace the slate-level exploration bonuses with the corresponding slot-level exploration bonuses, which results in a low per-round time complexity in Algorithms \ref{algo:batch_OFUL}, \ref{algo:TS} and \ref{algo:TS-Fixed}, while still exhibiting optimal regret guarantees. Details of the algorithm and the regret proof can be found in Sections \ref{section:main-algo}, \ref{section:TS} and Appendix \ref{appendix:ts-algos}. 

We would also like to highlight that many similar diversity assumptions have been studied throughout the literature, and several connections between these assumptions have been established (Section $3$, \cite{Papini2021}). Depending on the strength of the assumption, novel and stronger regret guarantees for well-known algorithms have been established (e.g., Lemma $2$, \cite{Papini2021} and Corollary $4$, \cite{Das_2024}). Interestingly, a core component of these regret proofs was also to show a linear lower bound on the minimum eigenvalue of the design matrix. Note that since the assumption is instance/algorithm-dependent, there may exist instances where this linear lower bound may not hold. To study this, we empirically examine the growth of the minimum eigenvalues ($\lambda_{\min}(\mathbf{W}_t^i)$) for a large number of randomly chosen instances. In all of the instances, we could clearly see a linear trend, thus validating the assumption, at least for these randomly picked instances. We refer the reader to Appendix \ref{appendix:empirical-validation} for more details on this empirical evaluation.



==> dtprsqbhrzmgzssxtywfnqcktqbmjtgr_5/arXiv_Sections_v2/Paper_Sections/other-experiments.tex <==
\section{Experiments}
\label{section:experiments}
In this section, we perform a wide range of synthetic (\textbf{Experiments 1,2,3})
% \footnote{The code can be found \href{https://github.com/sinhagaur88/Slate-Online-Logistic-Regression.git}{here}.} 
and real-world experiments (\textbf{Experiment 4})
% \footnote{The code can be found \href{https://github.com/tanmaygoyal258/Prompt_Optimization_Slate_Bandits.git}{here}.} 
to demonstrate the empirical performance of our algorithms \slateglincb, \slateglincbts\ and \slateglincbtsfixed. The codes for Experiments 1-3 and Experiment 4 can be found \href{https://github.com/tanmaygoyal258/Logistic_Slate_Bandits.git}{here} and \href{https://github.com/tanmaygoyal258/Prompt_Optimization_Slate_Bandits.git}{here} respectively. We now detail the setup for each of the experiments:


\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.33\columnwidth}  
		\centering 
		\includegraphics[width=56mm]{Plots/Finite_Contexts.pdf}
		\caption{{\small Regret vs.\ $T$: Finite Context Setting}}   
		\label{fig:finite-context-logistic}
	\end{subfigure}
	%\vskip\baselineskip
	\hfill
	\begin{subfigure}[b]{0.33\columnwidth}   
		\centering 
	\includegraphics[width=56mm]{Plots/Infinite_Contexts.pdf}
		\caption{{\small Regret vs.\ $T$: Infinite Context Setting}}   
		\label{fig:infinite-context-logistic}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.33\columnwidth}
		\centering
		\includegraphics[width=56mm]{Plots/non_contextual.pdf}
		\caption{{\small Regret vs.\ $T$: Fixed-Arm Setting}}     
		\label{fig:non-contextual-logistic}
	\end{subfigure}
	\vskip\baselineskip
	\begin{subfigure}[b]{0.33\columnwidth}  
		\centering 
		\includegraphics[width=56mm]{Plots/per_round_time_average.pdf}
		\caption{{\small Average running time (per-round)}}   
		\label{fig:average-time-per-round}
	\end{subfigure}
	%\vskip\baselineskip
	\hfill
	\begin{subfigure}[b]{0.33\columnwidth}   
		\centering 
		\includegraphics[width=56mm]{Plots/per_round_time_max.pdf}
				\caption{{\small Maximum running time (per-round)}}   
		\label{fig:maximum-time-per-round}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.33\columnwidth}
		\centering
		\includegraphics[width=56mm]{Plots/prompt_opt.pdf}
		\caption[observationalAlgo]%
        {{\small Accuracy vs.\ $T$: Prompt Optimization}}   
		\label{fig:prompt_opt}
	\end{subfigure}
	\caption{}
    \label{fig:Plots}
    %{\small Simple Regret} 
\end{figure*}

% \begin{figure*}
% 	\centering
% 	\begin{subfigure}[b]{0.65\columnwidth}  
% 		\centering 
% 		\includegraphics[width=56mm]{Plots/Finite_Contexts.pdf}
% 		\caption{{\small Regret vs.\ $T$: Finite Context Setting}}   
% 		\label{fig:finite-context-logistic}
% 	\end{subfigure}
% 	%\vskip\baselineskip
% 	\hfill
% 	\begin{subfigure}[b]{0.65\columnwidth}   
% 		\centering 
% 	\includegraphics[width=56mm]{Plots/Infinite_Contexts.pdf}
% 		\caption{{\small Regret vs.\ $T$: Infinite Context Setting}}   
% 		\label{fig:infinite-context-logistic}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.65\columnwidth}
% 		\centering
% 		\includegraphics[width=56mm]{Plots/non_contextual.pdf}
% 		\caption{{\small Regret vs.\ $T$: Fixed-Arm Setting}}     
% 		\label{fig:non-contextual-logistic}
% 	\end{subfigure}
% 	\vskip\baselineskip
% 	\begin{subfigure}[b]{0.65\columnwidth}  
% 		\centering 
% 		\includegraphics[width=56mm]{Plots/per_round_time_average.pdf}
% 		\caption{{\small Average running time (per-round)}}   
% 		\label{fig:average-time-per-round}
% 	\end{subfigure}
% 	%\vskip\baselineskip
% 	\hfill
% 	\begin{subfigure}[b]{0.65\columnwidth}   
% 		\centering 
% 		\includegraphics[width=56mm]{Plots/per_round_time_max.pdf}
% 				\caption{{\small Maximum running time (per-round)}}   
% 		\label{fig:maximum-time-per-round}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.65\columnwidth}
% 		\centering
% 		\includegraphics[width=56mm]{Plots/prompt_opt.pdf}
% 		\caption[observationalAlgo]%
%         {{\small Accuracy vs.\ $T$: Prompt Optimization}}   
% 		\label{fig:prompt_opt}
% 	\end{subfigure}
% 	\caption{}
%     \label{fig:Plots}
%     %{\small Simple Regret} 
% \end{figure*}


\textbf{Experiment 1 ($R(T)$ vs.\ $T$, Contextual Setting):}  In this experiment, we compare our algorithms \texttt{Slate-GLM-OFU} and \texttt{Slate-GLM-TS} to their counterparts \texttt{ada-OFU-ECOLog} (Algorithm 2, \cite{Faury2022}) and \texttt{TS-ECOLog} (Section D.2, \cite{Faury2022}). To the best of our knowledge, these are the only logistic bandit algorithms that achieve optimal ($\kappa$-free) regret, while simultaneously being computationally efficient, with a per-round time complexity of $O(\log^2 T)$. We experiment in the following two settings:
\begin{itemize}
    \item \textbf{Finite Contexts: } We assume the contexts come from the finite set $\C = \{1,\ldots,C\}$. For each $c\in \C$ and $i\in [N]$, before beginning the algorithm, a set of items $\X^{i,c}$ is constructed by randomly sampling $K$ vectors from the $d$-dimensional ball with radius $1/\sqrt{N}$ . Then, during the course of the algorithm, at each round $t$, a context $c$ is sampled uniformly at random from $\C$, and the sets $\X^{1,c}, \ldots , \X^{N,c}$ are presented to the learner.
    
    \item \textbf{Infinite Contexts: } At each
        round $t\in [T]$, and for each slot $i\in [N]$, set $\X_t^i$ is constructed by sampling $K$ vectors randomly from the $d-$dimensional ball with radius $1/\sqrt{N}$. The learner is then presented with $\{\X_t^i\}_{i \in [N]}$.
\end{itemize}
For the finite context setting, we fix $C=5$. For both settings, we fix the number of slots $N=3$, the number of items per slot $K=5$, and the dimension of item features $d=5$. To simulate the reward, we randomly sample $\bm\theta^\star$ from $[-1,1]^{15}$. We run our algorithms by varying the time horizon $T$ in $\{1000,5000,10000,15000, 20000\}$. For each $T$, we average the regret obtained at the end of $T$ rounds over 20 different seeds used to sample the rewards. The results for the Finite and Infinite context settings are shown in Figures \ref{fig:finite-context-logistic} and \ref{fig:infinite-context-logistic} respectively. In both instances, \texttt{Slate-GLM-OFU} performs the best, while \texttt{Slate-GLM-TS} performs on par with \texttt{TS-ECOLog}. Further, in Appendix \ref{appendix:experiments}, we report the average results with two standard deviations.

\textbf{Experiment 2 (Per-Round Time vs.\ $N$): }
In this experiment, we compare the average and maximum (per-round) time taken by our algorithms \texttt{Slate-GLM-OFU} and \texttt{Slate-GLM-TS}, with respect to their counterparts \texttt{ada-OFU-ECOLog} and \texttt{TS-ECOLog} \citep{Faury2022} respectively\footnote{The per-round time is calculated as the sum of the per-round pull and per-round update times.}. We record the per-round time taken by all algorithms while varying the number of slots $N$ in the set $\{3,\ldots , 6\}$. The number of items $(K = |\mathcal{X}^i_t|)$ per slot is fixed to $7$ and the dimension $d$ of each item is fixed to $5$. The item features are selected by randomly sampling from $[-1,1]^5$ and normalized to have norm $1/\sqrt{N}$. For each $N\in \{3,4,5,6\}$, we select a different reward parameter vector $\bm\theta^\star$ by randomly sampling from $[-1,1]^{5N}$. Note that the number of possible slates is $K^N$ and thus, varying $N$ in $\{3,4,5,6\}$ results in $343$, \;$2401$, \;$16807$, and $117649$ slates respectively. We perform this experiment in the infinite context setting (See \textbf{Experiment 1} for details). We run all the algorithms for $T = 1000$ rounds and average the results over 10 different seeds for sampling rewards. We show the average per-round running time in Figure \ref{fig:average-time-per-round} and the maximum per-round running time in Figure \ref{fig:maximum-time-per-round}. As expected, we observe much lower running times for \slateglincb\ and \slateglincbts\ compared to their counterparts. Moreover, the plots also indicate near-exponential growth in the per-round running time for both \texttt{ada-OFU-ECOLog} and \texttt{TS-ECOLog}. Further, there is a significant gap between the maximum and average per-round time of \texttt{Slate-GLM-OFU} and \texttt{Slate-GLM-TS}, implying that the actual per-round time for these algorithms is generally much lower than their maximum values. In Appendix \ref{appendix:experiments}, we report these results with two standard deviations. We also report the per-round time required to choose an arm, as well as, update parameters, separately, for each of our algorithms.

\textbf{Experiment 3 ($R(T)$ vs.\ $T$, Non-Contextual Setting):} In this experiment, we compare our algorithms \texttt{Slate-GLM-OFU}, \texttt{Slate-GLM-TS}, and \texttt{Slate-GLM-TS-Fixed} (Algorithm \ref{algo:TS-Fixed}, Appendix \ref{appendix:ts-algos}) to several state-of-the-art baseline algorithms, in the non-contextual setting, i.e., the set of candidate slates remains fixed throughout the course of the algorithm. 
Like previous experiments, our baselines include \texttt{ada-OFU-ECOLog} and $\texttt{TS-ECOLog}$ from \cite{Faury2022}. However, for the non-contextual setting, we also include other state-of-the-art baselines such as the \texttt{MPS} algorithm (Algorithm 3, \cite{Dimakopoulou2019}) and the \texttt{Ordered Slate Bandit} algorithm (Figure 3, \cite{Kale2010}). The latter is designed for semi-bandit feedback, and hence, we adapt it to the bandit feedback setting as explained in Appendix \ref{appendix:experiments}. We fix the number of slots $N$ to $3$ and the number of items in each slot $|\mathcal{X}^i_t| = K$ to $5$. The dimension $d$ of items for each slot is fixed to $5$. The items for each slot are randomly sampled from $[-1,1]^5$ and normalized to have norm $1/\sqrt{3}$, while $\thetastar$ is randomly sampled from $[-1,1]^{15}$ and normalized. We run all the algorithms for $T \in \{1000,5000,10000,20000,30000,40000,50000\}$ rounds and average the results over 50 different seeds for sampling rewards. The rewards are shown in Figure \ref{fig:non-contextual-logistic}. We see that \texttt{Slate-GLM-OFU} has the best performance, with the only algorithm having comparable performance being \texttt{MPS}. Also, \texttt{Slate-GLM-TS} performs worse than \texttt{ada-OFU-ECOLog} and \texttt{MPS} while being on par with \texttt{TS-ECOLog}. In Section \ref{appendix:experiments}, we showcase the average results with two standard deviations, which show that \texttt{MPS} showcases high variance, and hence, is less reliable in practice.


\textbf{Experiment 4 (Prompt Tuning):} In this experiment, we apply our contextual slate bandit algorithm \slateglincb\ to select in-context examples for tuning prompts of Language Models, applied to binary classification tasks. Typically, for such applications, a labeled training set of (input query, output label) pairs is used to learn policies of editing different parts of the prompt (such as instruction, in-context examples, verbalizers) \citep{Tempera2022} depending on a provided test input query. To simplify our task, we fix the instruction and the verbalizer and only select $N$ in-context examples from an available pool of $K$ examples. There are $N$ available positions (slots) in the prompt. Given a test input query (context), we create context-dependent features for the $K$ pool examples and independently select one (with repetition) per slot. This matches the contextual slate bandit problem setting (See Section \ref{section:preliminaries}) and therefore \slateglincb\ can be applied. We experiment on a sampled subset of size $5000$ from two popular sentiment analysis datasets, \emph{SST2} and \emph{Yelp Review}.  We randomly order the set and use about $\sim80\%$ ($4128$ for \emph{SST2}, $4000$ for \emph{Yelp Review}) of them for ``warm-up'' training and the remaining ~$20\%$ for testing. Like most prompt tuning experiments \citep{Tempera2022}, we report our results only on the test set; however, our algorithm continues to learn throughout the $5000$ rounds. The warm-up rounds help in obtaining a good estimate of the hidden reward parameter vector. We fix $N = 4$ and vary $K$ in the set $\cbrak{8,16,32}$. All the slots choose an example from the same $K$-sized example pool. At each round, given an input query $\bm{q}$ that needs to be solved for, item features for each in-context example $\bm{e}=(\bm{x}, y)$, is constructed by embedding each of $\bm{q}$, $\bm{x}$, and $y$ into 64 dimensions \citep{nussbaum2024nomic} and concatenating them, thereby resulting in a $192$-dimensional item feature vector. After selecting the $4$ items (slate), the resulting prompt (also containing the input query $\bm{q}$) is passed through the RoBERTa \citep{Zhuang2021} model and a possible answer for $\bm{q}$ is generated. Hence, we are learning to choose the best in-context examples for RoBERTa. At each round, we use GPT-3.5-Turbo to provide feedback (binary, $0$ or $1$) for the generated answer. This is treated as the reward for the chosen slate and utilized by the rest of the \slateglincb\ algorithm.
Figure \ref{fig:prompt_opt} shows the increase in cumulative accuracy as we sequentially proceed through the $5000$ data points in the \emph{Yelp Review} dataset. The data points to the left of the dotted blue line are the warm-up points, and those to the right are the test points. We can see that the cumulative accuracy increases consistently as we sequentially proceed through the points. Also, on the test set, the accuracy stays well above $80\%$.
We vary $K$ in the set $\{8,16,32\}$ and report the test accuracy for both datasets in Table \ref{table:prompt_opt}. It can be seen that the cumulative test accuracies for \slateglincb\ are much higher compared to the Random Allocation baseline, where each in-context example is chosen randomly (and hence, there is no learning). Also, we see that the accuracy generally increases when the pool size increases, potentially because of the availability of better examples. We do see a small decrease in accuracy when $K$ increases from $16$ to $32$ for the \emph{Yelp Review} dataset, and potentially attribute this dip to higher exploration.  


\begin{table}[H]
\centering
\def\arraystretch{1.0}%
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pool \\Size\end{tabular}} & \multicolumn{2}{c}{\textbf{SST2}}                                                                                                   & \multicolumn{2}{c}{\textbf{Yelp Review}}                                         \\ \cline{2-5} 
& \multicolumn{1}{c}{Random}            & \multicolumn{1}{c}{\texttt{Slate-GLM-OFU}}           & \multicolumn{1}{c}{Random}            & \multicolumn{1}{c}{\texttt{Slate-GLM-OFU}} \\ \hline
\multicolumn{1}{c}{8}           & \multicolumn{1}{c}{54.22}               & \multicolumn{1}{c}{69.15} & \multicolumn{1}{c}{62.90}               & \multicolumn{1}{c}{74.00} \\ 
\multicolumn{1}{c}{16}           & \multicolumn{1}{c}{54.46}               & \multicolumn{1}{c}{80.96} & \multicolumn{1}{c}{63.30}               & \multicolumn{1}{c}{82.50} \\ 
\multicolumn{1}{c}{32}           & \multicolumn{1}{c}{53.82}               & \multicolumn{1}{c}{81.42} & \multicolumn{1}{c}{62.00}               & \multicolumn{1}{c}{79.50} \\ \hline
\end{tabular}
}
\caption{Prompt Tuning Test Accuracy}
\label{table:prompt_opt}
\end{table}

==> dtprsqbhrzmgzssxtywfnqcktqbmjtgr_5/preamble.tex <==
% % \usepackage{mathtools}
% % \usepackage{amsfonts}
\usepackage{amssymb, amsmath}
\usepackage{xcolor}
\usepackage{amsthm}
% % \usepackage{enumitem}
% % %\usepackage[T1]{fontenc}
% % %\usepackage{mathpazo}
\usepackage{bm}
\usepackage{bbm}
% % %\usepackage{isomath}
% % \usepackage{verbatim}
% % \usepackage[dvipsnames,svgnames,table]{xcolor}
% % %\usepackage [english]{babel}
% % %\usepackage{charter}
% % \usepackage{bm}
% % \usepackage{bbold}
\usepackage{multirow}
% % \usepackage{enumerate}
% % \usepackage{caption}
%\usepackage{subcaption}
%\usepackage{subfigure}
\usepackage{graphicx}
\usepackage{subcaption}
% % \usepackage{mathrsfs}
% % \usepackage{bbm}
% % %\usepackage{mathabx}
% % %\usepackage[utf8]{inputenc}
% % %\usepackage{cite}
% % \usepackage{hyperref}
% % %\usepackage{pslatex}
% % %packaged for figures
% % \usepackage{tikz}
% % %\usetikzlibrary{positioning}
% % \usetikzlibrary{calc}
% % %\usetikzlibrary{decorations.shapes}
% % %\usetikzlibrary{decorations.pathreplacing,angles,quotes}

%\usepackage{algorithmicx,algorithm}
% % % \usepackage{algpseudocode}
% % \usepackage{natbib}
\usepackage{algorithmic, algorithm}
% % \usepackage{cleveref}




% %paragrpah spacing
% %\setlength{\parindent}{2em}
% %\setlength{\parskip}{1em}

% %importing packages
% %\usepackage{fullpage}


% %custom theorem labelling
% \newtheorem{innercustomthm}{Theorem}
% \newenvironment{customthm}[1]
%   {\renewcommand\theinnercustomthm{#1}\innercustomthm}
%   {\endinnercustomthm}

% %for colored links
% \definecolor{blueviolet}{RGB}{60,50,200}
% \definecolor{oliveg}{RGB}{40,200,30}
% \hypersetup{colorlinks=true,       % false: boxed links; true: colored links
%     linkcolor=blueviolet,
%     citecolor=oliveg,
% }


% %\usepackage{algpseudocode}
% % \usepackage[ruled]{algorithm2e}

% %\usepackage{stmaryrd}

% %Suggested by ECCC
% %\usepackage{color}
% %\usepackage[pdfstartview=FitH,pdfpagemode=None,colorlinks=true,citecolor=blue,linkcolor=magenta]{hyperref}
% %END Suggested by ECCC

% %\usepackage{palatino}
% %\usepackage{complexity}
% %\usepackage{todonotes}

% %new counter for theorem
% %\newcounter{counttheorem}

% % defining new environment
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{problem}{Problem}
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{fact}{Fact}
\newtheorem{thm}{Theorem}[theorem]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{subclaim}{Subclaim}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{assumption}{Assumption}[section]
% %defining new commands
% %\newcommand{\SUM}[2]{\sum_{#1}^{#2}}
% % \newtheorem{theorem}{Theorem}[section] % theorems will be numbered according to section
% % \newtheorem{lemma}[theorem]{Lemma} % lemmas share the counter with theorems
% % \newtheorem{cor}[theorem]{Corollary} % ditto


% \newcommand{\StateGLinCB}{\texttt{StateGLinCB}\xspace}

% %footnotes
% %\renewcommand\thefootnote{\textcolor{red}{\arabic{footnote}}}
% %\makeatletter
% %\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
% %\makeatother

% \makeatletter
% \newcommand{\printfnsymbol}[1]{%
%   \textsuperscript{\@fnsymbol{#1}}%
% }
% \makeatother

% %for algorithm removing colon
% %\algsetup{linenodelimiter=.}



% % \newtheorem{example}{Example}[section]

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}



\newcommand{\slateglincb}{\texttt{Slate-GLM-OFU}}
\newcommand{\slateglincbts}{\texttt{Slate-GLM-TS}}
\newcommand{\slateglincbtsfixed}{\texttt{Slate-GLM-TS-Fixed}}
\newcommand{\adaofuecolog}{\texttt{ada-OFU-ECOLog}}
\newcommand{\tsecolog}{\texttt{TS-ECOLog}}

\def\DEBUG{true} % set this to be false to remove comments
\ifdefined\DEBUG
% 	    \newcommand{\vineet}[1]{\textcolor{Red}{#1}}
% 	    \newcommand{\vishakha}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\gaurav}[1]{\textcolor{red}{[Gaurav:#1]}}
% 	    \def\rem#1{{\marginpar{\raggedright\scriptsize #1}}}
% 	    \newcommand{\vin}[1]{\rem{\textcolor{Red}{$\bullet$ #1}}}
% 	    \newcommand{\vis}[1]{\rem{\textcolor{OliveGreen}{$\bullet$ #1}}}
% 	    \newcommand{\gau}[1]{\rem{\textcolor{NavyBlue}{$\bullet$ #1}}}
\else
% 	    \newcommand{\vineet}[1]{#1}
% 	    \newcommand{\vishakha}[1]{#1}
 	    \newcommand{\gaurav}[1]{}
%         \newcommand{\vin}[1]{}
% 	    \newcommand{\vis}[1]{}
% 	    \newcommand{\gau}[1]{}
	 
\fi



% % added by Tanmay
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\ddash}{p}
\newcommand{\E}{\mathbb{E}}
\newcommand{\C}{\mathcal{C}}
\renewcommand{\H}{\mathcal{H}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\event}{\mathcal{E}}
% \newcommand{\x}{\bm{x}}
% \renewcommand{\theta}{\bm{\theta}}
\newcommand{\eventc}[1]{\overline{#1}}


% % filteration
\newcommand{\filteration}[1]{\mathcal{F}_{#1}}

% % transpose and inverse
\newcommand{\T}{^T}
\newcommand{\inv}{^{-1}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}
% % eigenvalues
\newcommand{\eigmax}[1]{\lambda_{\max}\left(#1\right)}
\newcommand{\eigmin}[1]{\lambda_{\min}\left(#1\right)}

% % singular values
\newcommand{\singmax}[1]{\sigma_{\max}\left(#1\right)}
\newcommand{\singmin}[1]{\sigma_{\min}\left(#1\right)}

% % inequalities
\newcommand{\mleq}{\preccurlyeq}
\newcommand{\mgeq}{\succcurlyeq}

% % norms
\newcommand{\twonorm}[1]{\left\Vert#1\right\Vert_2}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\matnorm}[2]{\left\Vert#1\right\Vert_{#2}}


% % brackets
\newcommand{\sbrak}[1]{\left[#1\right]}
\newcommand{\pbrak}[1]{\left(#1\right)}
\newcommand{\cbrak}[1]{\left\{#1\right\}}
\newcommand{\modulus}[1]{\left|#1\right|}

% %optimal params
\newcommand{\thetastar}{\bm{\theta}_\star}

% % inner product and expected reward
\newcommand{\inner}[2]{#1^\intercal#2}
\newcommand{\exprew}[2]{\mu\pbrak{\inner{#1}{#2}}}

% % sum
\newcommand{\summation}[2]{\sum\limits_{#1}^{#2}}

% % sigmoid
\newcommand{\sigmoid}[1]{\mu\pbrak{#1}}
\newcommand{\dsigmoid}[1]{\dot{\mu}\pbrak{#1}}
\newcommand{\sens}[2]{\dot{\mu}\pbrak{\inner{#1}{#2}}}


% % diameter
\newcommand{\diam}[2]{\text{diam}_{#1}\pbrak{#2}}
